An extended discontinuous Galerkin shock tracking method

In this paper, we introduce a novel high-order shock tracking method and provide a proof of concept. Our method leverages concepts from implicit shock tracking and extended discontinuous Galerkin methods, primarily designed for solving partial differential equations featuring discontinuities. To address this challenge, we solve a constrained optimization problem aiming at accurately fitting the zero iso-contour of a level set function to the discontinuities. Additionally, we discuss various robustness measures inspired by both numerical experiments and existing literature. Finally, we showcase the capabilities of our method through a series of two-dimensional problems, progressively increasing in complexity.

==> Bibliography.tex <==
\begin{thebibliography}{99}
%\bibitem{muller2016} Müller, B., Krämer‐Eis, S., Kummer, F., Oberlack, M., 2017. A high-order discontinuous Galerkin method for compressible flows with immersed boundaries. International Journal for Numerical Methods in Engineering 110, 3–30.

%\bibitem{geisenhofer2019} Geisenhofer, M., Kummer, F., Müller, B., 2019. A discontinuous Galerkin immersed boundary solver for compressible flows: Adaptive local time stepping for artificial viscosity–based shock-capturing on cut cells. International Journal for Numerical Methods in Fluids 91, 448–472.

%\bibitem{salas2010} Salas, M.D., 2010. A shock-fitting primer, Chapman \& Hall/CRC applied mathematics and nonlinear science series. CRC Press, Boca Raton.

%\bibitem{kummer2016} Kummer, F., 2016. Extended discontinuous Galerkin methods for two-phase flows: the spatial discretization. International Journal for Numerical Methods in Engineering 109, 259–289.
\bibitem{Anderson} John D. Anderson Jr. , 2003 Modern Compressible Flow 3th Edition
\bibitem{Geisenhofer} Markus C. Geisenhofer, 2020 From Shock-Capturing to
High-Order Shock-Fitting
\bibitem{XDG} Kummer, Smuda, Weber, 2020 BoSSS: a package for multigrid extended discontinuous Galerkin methods
\bibitem{ZahrHOIST} Zahr, H., 2021 A robust, high-order implicit shock tracking method for simulation of complex, high-speed flows, http://arxiv.org/abs/2105.00139
\bibitem{Corrigan MDG-ICE} Andrew Corrigan Andrew D. Kercher David A. Kessler, 2019  A moving discontinuous Galerkin finite element method for flows with interfaces

\bibitem{PersonPerraire} Per-Olof Persson, Jaime Peraire, 2006 Sub-cell shock capturing for discontinuous Galerkin methods, AIAA Paper 2006-112.



\end{thebibliography}

==> babelbst.tex <==
% Language setting for diss_harv_babel.bst
%
% INPUT ONE LANGUAGE FILE ONLY !
%
% read one of the files germbst.tex or englbst.tex
% for further information
%
% When using harvard.sty, this file has to be included in the main
% document file with the '\input' command. Otherwise, repeated
% citations will not work properly since then the \bbl... commands
% are unknown commands in the main file.
%\input germbst.tex
 \input englbst.tex


==> englbst.tex <==
%% This file was renamed to englbst.tex from babelbst.tex
%%
%%
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% IMPORTANT NOTICE:
%%
%% For the copyright see the source file.
%%
%% Any modified versions of this file must be renamed
%% with new filenames distinct from babelbst.tex.
%%
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%%
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2005 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2005/10/17 4.14 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}                \def\bbletal{et~al.}
\def\bbleditors{editors}        \def\bbleds{eds.}
\def\bbleditor{editor}          \def\bbled{ed.}
\def\bbledby{edited by}
\def\bbledition{edition}        \def\bbledn{edn.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{of}
\def\bblnumber{number}          \def\bblno{no.}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapter}        \def\bblchap{chap.}
\def\bbltechreport{Technical Report}
\def\bbltechrep{Tech. Rep.}
\def\bblmthesis{Master's thesis}
\def\bblphdthesis{Ph.D. thesis}
\def\bblfirst{First}            \def\bblfirsto{1st}
\def\bblsecond{Second}          \def\bblsecondo{2nd}
\def\bblthird{Third}            \def\bblthirdo{3rd}
\def\bblfourth{Fourth}          \def\bblfourtho{4th}
\def\bblfifth{Fifth}            \def\bblfiftho{5th}
\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}
\def\bblth{th}
\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}
\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}
\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}
\endinput
%%
%% End of file `babelbst.tex'.

